Monte-Carlo Tree Search for Policy Optimization

Gradient-based methods are often used for policy optimization in deep reinforcement learning, despite being vulnerable to local optima and saddle points. Although gradient-free methods (e.g., genetic algorithms or evolution strategies) help mitigate these issues, poor initialization and local optima are still concerns in highly nonconvex spaces. This paper presents a method for policy optimization based on Monte-Carlo tree search and gradient-free optimization. Our method, called Monte-Carlo tree search for policy optimization (MCTSPO), provides a better exploration-exploitation trade-off through the use of the upper confidence bound heuristic. We demonstrate improved performance on reinforcement learning tasks with deceptive or sparse reward functions compared to popular gradient-based and deep genetic algorithm baselines.

==> macros.tex <==
\usepackage{cleveref}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
\usepackage{acronym}
%\usepackage{color,xcolor}
\usepackage{verbatim}
\usepackage{booktabs}
\usepackage{siunitx}
\usepackage{graphicx,caption}
\usepackage{amsmath,amssymb,stmaryrd,mathtools}
\usepackage[keeplastbox]{flushend}
\usepackage{graphics}
% \usepackage{subcaption}
\usepackage{suffix}
\usepackage{xstring}
\usepackage{xparse}
\usepackage{expl3}

% \usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{amsmath}
\usepackage{tikz}
\usetikzlibrary{arrows,backgrounds,calc}
\usepackage{relsize}

%% PGF preamble
\RequirePackage{luatex85}
% \documentclass[tikz]{standalone}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\pgfplotsset{every axis legend/.append style={%
		cells={anchor=west}}
}
\usepgfplotslibrary{polar}
\usetikzlibrary{arrows}
\tikzset{>=stealth'}

\definecolor{C1}{rgb}{0.0, 0.447, 0.741}
\definecolor{C1_light}{rgb}{0.0, 0.6032388663967612, 1.0}
\definecolor{C2}{rgb}{0.85, 0.325, 0.098}
\definecolor{C3}{rgb}{0.929, 0.694, 0.125}
\definecolor{C4}{rgb}{0.494, 0.184, 0.556}
\definecolor{C5}{rgb}{0.466, 0.674, 0.188}
\definecolor{C6}{rgb}{0.301, 0.745, 0.933}
\definecolor{C7}{rgb}{0.635, 0.078, 0.184}

\usepgfplotslibrary{groupplots}

\usetikzlibrary{shapes.geometric, arrows}

\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=2cm, minimum height=1cm,text centered, draw=black, fill=none]
\tikzstyle{arrow} = [thick,->,>=stealth]

% *** ALIGNMENT PACKAGES ***
\usepackage{array}
% The following packages can be found on http:\\www.ctan.org
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{bbold}
\usepackage{siunitx}
\usepackage{subfig}
% \usepackage{subcaption}
% tables
\usepackage{multirow}

%%
\usepackage{suffix}
\usepackage{xstring}
\usepackage{xparse}
\usepackage{expl3}

\usepackage{url}
\usepackage{dsfont}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{acronym}
\usepackage{color,xcolor}
\usepackage{verbatim}
\usepackage{booktabs}
\usepackage{siunitx}
\usepackage{graphicx,caption}
\usepackage{amsmath,amssymb,stmaryrd,mathtools}
\usepackage[keeplastbox]{flushend}
% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}

% *** CITATION PACKAGES ***
%\usepackage{cite}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{acronym}
\usepackage{color,xcolor}
\usepackage{verbatim}
\usepackage{booktabs}

\newcommand{\norm}[1]{\left\lVert #1 \right\rVert} % http://tex.stackexchange.com/questions/70020/how-to-write-euclidean-distance
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert} % http://tex.stackexchange.com/questions/70020/how-to-write-euclidean-distance

\graphicspath{{./figures/}}

%argmin
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\ignore}[1]{}
%\newcommand{\comment}[1]{{\color{red} #1 }}
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
%\newtheorem{proof}{Proof}[section]

\newcommand{\eg}{e.\,g.,\ }
\newcommand{\ie}{i.\,e.,\ }
\newcommand{\etal}{{et~al.}}

%introduce \powerset - hint by http://matheplanet.com/matheplanet/nuke/html/viewtopic.php?topic=136492&post_id=997377
\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
  <6-7>  MnSymbolC6
  <7-8>  MnSymbolC7
  <8-9>  MnSymbolC8
  <9-10> MnSymbolC9
 <10-12> MnSymbolC10
 <12->   MnSymbolC12%
}{}
\DeclareMathSymbol{\powerset}{\mathord}{MnSyC}{180}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% this package is for todo notes!
%===todonotes====
\usepackage{todonotes}
\usepackage{soul}
\definecolor{smoothgreen}{rgb}{0.7,1,0.7}
\sethlcolor{smoothgreen}

\newcommand{\todopara}[1]{\vspace{0px} %
\todo[inline, color=black!10]{\textbf{[Paragraph:]} {#1}} %
}
\newcommand{\todonote}[1]{\vspace{0px} %
\todo[inline, color=green!30]{\textbf{[Note:]} {#1}} %
}
\newcommand{\todoQ}[1]{\vspace{0px} %
\todo[inline, color=orange!50]{\textbf{[Note:]} {#1}} %
}
\newcommand{\todohere}[1]{\hl{(\textbf{TODO:} #1)}}

\newcommand{\hidetodos}{
\renewcommand{\todopara}[1]{}
\renewcommand{\todonote}[1]{}
\renewcommand{\todoQ}[1]{}
\renewcommand{\todohere}[1]{}}
%\hidetodos
%===end todonotes===

\newcommand{\citet}[1]{\citeauthor{#1}~\shortcite{#1}}
